Fast Computation of Empirically Tight Bounds for the Diameter of Massive Graphs

The diameter of a graph is among its most basic parameters. Since a few years, it moreover became a key issue to compute it for massive graphs in the context of complex network analysis. However, known algorithms, including the ones producing approximate values, have too high a time and/or space complexity to be used in such cases. We propose here a new approach relying on very simple and fast algorithms that compute (upper and lower) bounds for the diameter. We show empirically that, on various real-world cases representative of complex networks studied in the literature, the obtained bounds are very tight (and even equal in some cases). This leads to rigorous and very accurate estimations of the actual diameter in cases which were previously untractable in practice.

==> vire <==
So, as the paper is an empirical study I feel it could investigate the subject more thoroughly and give more detailed analysis of performance and biases of various bounds and make more explicit suggestions to practitioners who want to calculate the diameter of massive graphs.


-- section 1, 4th paragraph: the D do not print well: it says "to an estimation D of D such that D \le D \le D+2. I guess you want some bars or hats. :)
-- similarly table 1 prints without lines which makes it hard to read.


